Scene Understanding for Autonomous Driving

To detect and segment objects in images based on their content is one of the most active topics in the field of computer vision. Nowadays, this problem can be addressed using Deep Learning architectures such as Faster R-CNN or YOLO, among others. In this paper, we study the behaviour of different configurations of RetinaNet, Faster R-CNN and Mask R-CNN presented in Detectron2. First, we evaluate qualitatively and quantitatively (AP) the performance of the pre-trained models on KITTI-MOTS and MOTSChallenge datasets. We observe a significant improvement in performance after fine-tuning these models on the datasets of interest and optimizing hyperparameters. Finally, we run inference in unusual situations using out of context datasets, and present interesting results that help us understanding better the networks.

==> tables/w4/old.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{ccccccc}
\toprule
Architecture & \multicolumn{2}{c}{{FasterRCNN}} & \hspace{0.1cm} & \multicolumn{2}{c}{RetinaNet}\\ 
 \cmidrule{2-3} 
 \cmidrule{5-6} 
AP & Pretrained & Finetuned && Pretrained & Finetuned \\ 
\midrule
Mean & 55.61 & 60.31 && 56.63 & 61.47 \\
Car & 65.72 & 66.93 && 67.14 & 67.84 \\
Pedestrian & 45.50 & 53.69 && 46.13 & 55.1 \\
\bottomrule
\end{tabular}
\caption{Comparison of results before and after fine-tuning our model on the KITTI MOTS and MOTSChallenge datasets}
\label{tab:after_finetune}
\end{table}


\begin{table}[b!]
\centering
\begin{tabular}{c|cccc|c}
\toprule
Batch(ROI) & 0 & 1 & 2 & 3 & Mean AP \\
\midrule
\textbf{256} & \textbf{58.01} & \textbf{64.60} & \textbf{62.01} & \textbf{69.94} & \textbf{63.64} \\
512 & 57.81 & 63.97 & 62.08 & 68.49 & 63.09 \\
1024 & 55.54 & 62.44 & 61.12 & 67.79 & 61.72 \\
\bottomrule
\end{tabular}
\caption{mAP for cross-val split for Model: faster\_rcnn\_R\_50\_FPN\_3x}
\label{tab:faster_hyper_batch}
\end{table}


\begin{table}[t!]
\centering
\begin{tabular}{c|cccc|c}
\toprule
LR & 0 & 1 & 2 & 3 & Mean AP \\
\midrule
1e-3 & 57.39 & 61.13 & 62.05 & 69.73 & 62.58 \\
1e-4 & \textbf{57.81} & \textbf{63.97} & \textbf{62.08} & \textbf{68.49} & \textbf{63.09} \\
1e-5 & 55.27 & 62.21 & 59.44 & 65.36 & 60.57 \\
\bottomrule
\end{tabular}
\caption{mAP for cross-val split for Model: faster\_rcnn\_R\_50\_FPN\_3x}
\label{tab:faster_hyper_lr}
\end{table}


\begin{table}[b!]
\centering
\begin{tabular}{cccc}
\toprule
 & \multicolumn{3}{c}{{Model: retinanet\_}} \\ 
\cmidrule{2-4} 
Metric & R50-FPN-1X & R50-FPN-3X & R101-FPN-3X \\ 
\midrule
AP   & 55.31 & \textbf{56.63} & 55.19 \\
APs  & 28.63 & \textbf{29.92} & 28.87 \\
APm  & 61.36 & \textbf{62.75} & 60.25 \\
APl  & 72.26 & \textbf{73.13} & 74.01 \\
\bottomrule
\end{tabular}
\caption{Pre-trained RetinaNet Models evaluated on the KITTI MOTS validation dataset}
\label{tab:retina_pre_trained}
\end{table}

\begin{table*}[t!]
\centering
\begin{tabular}{ccccccc|ccc}
\toprule
 & \multicolumn{9}{c}{{Model: FasterRCNN\_}} \\ 
\cmidrule{2-10}
& \multicolumn{6}{c|}{{R-50-X}} & \multicolumn{3}{c}{{R-101-X}}  \\
Metric & C4-1x & DC5-1x & FPN-1x & C4-3x & DC5-3x & FPN-3x & C4-3x & DC5-3x & FPN-3x \\ 
\midrule
AP   & 53.08 & 51.15 & 54.83 & 53.65 & 52.62 & \textbf{55.61} & 54.15 & 54.48 & 56.44 \\
APs  & 23.78 & 24.23 & 29.26 & 24.58 & 25.32 & \textbf{30.21} & 26.52 & 25.81 & 30.46 \\
APm  & 59.33 & 56.28 & 60.50 & 59.86 & 57.51 & \textbf{61.20} & 59.46 & 60.06 & 61.50 \\
APl  & 71.71 & 69.90 & 70.82 & 71.72 & 71.10 & \textbf{70.40} & 73.03 & 74.24 & 73.06 \\
\bottomrule
\end{tabular}
\caption{Pre-trained FasterRCNN Models evaluated on the KITTI MOTS validation dataset}
\label{tab:fasterrcnn_pre_trained}
\end{table*}

